IcebergHT: High Performance PMEM Hash Tables Through Stability and Low Associativity

Modern hash table designs strive to minimize space while maximizing speed. The most important factor in speed is the number of cache lines accessed during updates and queries. This is especially important on PMEM, which is slower than DRAM and in which writes are more expensive than reads. This paper proposes two stronger design objectives: stability and low-associativity. A stable hash table doesn't move items around, and a hash table has low associativity if there are only a few locations where an item can be stored. Low associativity ensures that queries need to examine only a few memory locations, and stability ensures that insertions write to very few cache lines. Stability also simplifies scaling and crash safety. We present IcebergHT, a fast, crash-safe, concurrent, and space-efficient hash table for PMEM based on the design principles of stability and low associativity. IcebergHT combines in-memory metadata with a new hashing technique, iceberg hashing, that is (1) space efficient, (2) stable, and (3) supports low associativity. In contrast, existing hash-tables either modify numerous cache lines during insertions (e.g. cuckoo hashing), access numerous cache lines during queries (e.g. linear probing), or waste space (e.g. chaining). Moreover, the combination of (1)-(3) yields several emergent benefits: IcebergHT scales better than other hash tables, supports crash-safety, and has excellent performance on PMEM (where writes are particularly expensive).

==> Makefile <==
ALL = main.pdf
TEXFILES = main abstract defines includes intro title pmem experiments plots plot-micro-pmem plot-ycsb-pmem plot-micro-dram plot-ycsb-dram plot-latency plot-histo multithreading iceberg impl resizing discussion related
FIGURES =
LATEXMKOPTS = -pdf -dvi-
LATEX = pdflatex
BIBFILES = bibliography

########### Shouldn't require configuration below here ##########

# run "make CONT=1" for continuous compilation
ifdef CONT
	LATEXMKOPTS += -pvc
	FORCED = .PHONY
endif

all: $(ALL)

$(ALL): $(TEXFILES:=.tex) $(FIGURES) $(BIBFILES:=.bib)

# How to compile a .tex file to a .pdf file
%.pdf: %.tex $(FORCED)
	@if (command -v latexmk > /dev/null) ; then latexmk $(LATEXMKOPTS) $< ; \
	else $(LATEX) $<; bibtex $@; $(LATEX) $<; $(LATEX) $<; fi 

#
# Rules for converting various figure formats to pdf
#

%.pdf_tex: %.svg
	inkscape -A $(@:.pdf_tex=.pdf) --export-latex $<

%.pdf: %.svg
	inkscape -A $@ $<

%.pdf: %.dia
	dia --nosplash -e $(@:.pdf=.eps) $(@:.pdf=.dia) 
	epstopdf $(@:.pdf=.eps)

%.pdf: %.fig
	fig2dev -L pdftex $< $@

%.pdf_t: %.fig %.pdf
	fig2dev -L pdftex_t -p $(@:.pdf_t=.pdf) $< $@

%.pstex_t: %.fig
	fig2dev -L pstex_t -p $(@:.pstex_t=.pstex) $< $@
	fig2dev -L pstex $< $(@:.pstex_t=.pstex)

.PHONY:

clean:
	latexmk -C


==> backups/abstract.tex <==
% !TEX root =  main.tex

\begin{abstract}
%

Persistent memory (PMEM) poses two new challenges that are not seen with DRAM---\emph{crash consistency} and \emph{read-write-performance asymmetry}. 
These challenges have led researchers to completely redesign hash tables and other software systems around the performance characteristics and crash consistency requirements of PMEM.
% MAB: topic of paragraph: the conventional wisdom is wrong
%The conventional wisdom is that an algorithm or data structure that is optimized for one technology will run inefficiently on the other.
This paper demonstrates that, at least for hash tables, the conventional wisdom---that separate designs are needed for high performance in DRAM and PMEM---is wrong. 

% MAB: topic of paragraph: I stability and associativity get both, and what they are.
We begin by identifying two properties of hash tables, \emph{stability} and \emph{low associativity}, that when achieved simultaneously can result in strong
performance in both DRAM and PMEM while simultaneously removing most of the difficulties in achieving crash consistency.
A hash table is \defn{stable} if it guarantees that the position where an element is stored will not change until either the element is deleted or the table is resized.
\mab{Maybe mention that stability helps  PMEM in an additional way because writes are expensive in PMEM.}
A hash table has  \defn{low associativity} if the maximum number of locations where an element is permitted to reside is small. 
% Cuckoo hashing is the canonical example of a low-associative hash table, but it isn't stable, whereas a chained hash table is stable, but does not have low associativity.
There is a tension between these two properties, and existing hash tables achieve at most one of these properties. 
% , and most existing hash tables have at most one of these two properties. 








We present a new hash table, \sysname, that has both. It has low associativity since it accesses a small, constant number of cache lines for both queries and updates and modifies only a single cache line per update.
%
Moreover, \sysname is stable, which 
% , i.e., no item gets moved after it is inserted, except when the hash table is resized. 
not only improves write performance, but  also permits a very simple, nearly lock-free design, yielding  high concurrency. 
%
The result is that achieving crash-safety becomes trivial.  Stability also  eliminates the need
for fences, because inserts only modify the slot of the inserted item.

\mab{this is a sentence that should be deleted or better incorporated. As is, it doesn't help
  ``The key idea behind \sysname is to reduce the associativity of stable hash
tables, and then keep enough metadata in RAM to record each
item's exact location.''}

We evaluated \sysname both in DRAM and in PMEM.
In DRAM, \sysname runs about $2\times$ faster than libcuckoo and between
$2\times$ and $9\times$ faster than TBB.  In PMEM, \sysname runs
about 10\% to 80\% faster than Dash. \Sysname also exhibits nearly linear
scaling with the number of threads across all workloads we evaluated, both in
 DRAM and in PMEM.
%
\end{abstract}

%%%%%%% Notes %%%%%%%%%%%%%%

%\begin{verbatim}
%There are very different performancwe characterstiucs b/w DRAM and PMEM
%this suggests different data str design

%- asymetry 
%- crash consistency
%- slower access cost

%These significant differences have prompted rersearchers to redesign data
%structures for PMEM

%It's also the case that hash tables are designed for specific for specific
%operations
%- cuckoo for queries
%- chaining for crash consistency

%This also suggests there is a whole range of design choices


%This paper makes a surprise claim that this is not true.
%We identify two properties that are given you different goodnesses
%- Stability
%- Low associativity

%The reason that there have been many designs because of different hardware and
%operations.. is that no hash table both these featurs together or at the same
%time

%e.g., cuckoo low associativity but not stable
%chaining has stable but igh associativity

%We present Iceberg HT ... achieves both... stability and low associativity
%Consequence...

%- Faster across hardware, DRAM and PMEM
%- Faster across operations/workloads
%- Great scalability with increasing threads.....





%People have said to completely redeisgn data structures for PMEM due to
%two differences between DRAM and PMEM

%- crash safety
%- radically diffferent performance model

%But here we show that it not true for hash tables
%design techniques for hash tables 
%it enables us to treat PMEM as a slow DRAM
%Good performance in DRAM and same in PMEM
%Crash safety comes for free
%and concurrency also comes for free


%These results are promising to suggest that we can extend this for other data
%structures....


%basically, nvm is similar just slower
%a good ds for RAM is also for PMEM

%a new dats str.. making crash safety problem trivial
%moreover, it makes concurrency also simple

%\end{verbatim}




%%%%%%%%%%%%%% Old abstract %%%%%%%%%
%Hash table performance on modern hardware is primarily determined by the number
%of cache lines accessed during queries and updates. For updates, it is also
%important to minimize the number of cache lines modified by the update,
%especially when the hash table lives in persistent memory, where writes are
%particularly slow. Traditional hash tables, such as chained, linear probing,
%and quadratic probing, access up to $O(\log n)$ cache lines for inserts and
%queries and modify only 1 cache line.
%%
%%\mab{Martin and I have concerns about the sentence, and will deal with it when
  %%it turns out to be the highest nail.}
%%
%Several modern hash table designs, such as cuckooing and Robin Hood, reduce the
%number of cache lines accessed during queries but increase the number of cache
%lines dirtied by updates.

%This paper presents a new hash table, \sysname, that accesses a small, constant
%number of cache lines on both queries and updates and modifies only a single
%cache line per update.
%%
%In fact, \sysname is \emph{stable}, i.e., no item gets moved after it is inserted,
%except when the hash table is resized. 
%%
%Stability not only improves performance, it yields high concurrency with a very
%simple, nearly lock-free design.
%%
%And, on persistent memory, it makes crash-safety easy and eliminates the need
%for fences, because inserts modify only the slot of the inserted item.

%The key idea behind \sysname is to reduce the \emph{associativity}, i.e., the
%number of locations in which an item can be stored, of stable hash tables to
%$O(\log n)$, and then keep enough metadata in RAM to record each item's exact
%location.

%In DRAM, \sysname is generally about $2\times$ faster than libcuckoo and between
%$2\times$ and $9\times$ faster than TBB.  In persistent memory, \sysname is
%about 10\% to 80\% faster than Dash. \Sysname also exhibits nearly linear
%scaling with increasing number of threads across all workloads we evaluated in
%both DRAM and persistent memory.




==> backups/implement.tex <==
% !TEX root =  main.tex

\section{\Sysname}\label{sec:design}


\begin{figure}[t]
  \centering
  \resizebox{\columnwidth}{!}{%
  \includegraphics{iceberg_table}
}
  \caption{\boldmath Iceberg hash table block structure. Iceberg table has three levels.
  To insert a key value pair, we first hash the key $h_0(\mbox{key})$ and
  determine a block in level 1.
  %
  If the block in level 1 is full, we try to insert it in level 2. In level 2,
  we hash the key twice $h_1(\mbox{key})$ and $h_2(\mbox{key})$ and insert the
  key in the emptier block.
  %
  If the both blocks are full in level 2 then we insert the key value pair in
  level 3 block $h_0(\mbox{key})$.}
  \label{fig:iceberg_table}
\end{figure}


In this section, we first describe how to design a hash table based on
Iceberg hashing; see \Cref{sec:theory}. We later give an
overview of how to perform operations in \sysname.

The \sysname hash table consists of three levels 
(see \Cref{fig:iceberg_table}). The first level acts as the front
yard where most of the key-value pairs are stored. The level is divided
into blocks, where each block has 64 slots to store key-value pairs.  We use a
single hash function $h_0(x)$ to determine a block in level 1 to store the
key-value pair. 

The second and the third level act as the backyard. The second level is much
smaller in size ($12.5\%$) compared to the first level. It is also divided
into blocks and consists of the same number of blocks as the first level but
each block only has 8 slots to store key-value pairs. We use power-of-two-choice
hashing to determine the block to store a key in level 2. In power-of-two-choice
hashing, a key is hashed to two blocks ($h_1(x)$ and $h_2(x)$) and placed in the
emptier block.

The third level consists of an array of linked lists. Keys that do not find an
empty slot in level 2 due to full capacity are stored in this level. The size of
the array in the third level is the same as the number of blocks in level 1 and
2. We use the same hash function as used in level 1 ($h_0(x)$) to determine a
linked list to add the key-value pair. 

The third level is mostly empty (<{}<1\% please refer to~\Cref{tab:key-dist}) for
all practical hash table configurations (i.e., when the hash table capacity is
$<95\%$) and therefore the choice of structure has little effect on performance.

\subsection{Metadata scheme}
\mabinline{It feels as though we need a punchier topic sentence(s) for the subsection. The material is exciting, but the exciting part is buried. 
E.g.,  the metadata scheme takes advantage of vector operations so that for level 1, there's one memory access to the metadata and one to level 1. Or something similar.}

One of the impediments to storing key-value pairs in large buckets as in
\sysname is that large buckets span multiple cache lines. This hurts the cache
efficiency, because operations may need to access multiple cache lines per
block.

\sysname addresses this concern by storing metadata for each block, consisting
of an 8-bit fingerprint for each slot. If the slot holds a valid key, the
fingerprint is a hash of the key, otherwise it holds one of two special values:
\texttt{EMPTY} or \texttt{RESERVED}. This latter value is used for
synchronization, see \Cref{multithreading}.

The metadata scheme thus has a space overhead of 6.25\% for a 16 byte key-value
pair.  Importantly, because the blocks in level 1 have 64 slots and the blocks
in level 2 have 8 slots, the metadata for each block fits in a single cache
line.

During an insert operation, probing the metadata corresponding to a block
indicates which slots are empty in the block. The insert can then try insert
the new key into one of those empty slots.

During a query operation, the fingerprint of the queried key can be checked
against the fingerprints in the metadata, yielding only those slots with a
matching fingerprint. This filters out empty slots as well as nearly all slots
with non-matching keys.

The metadata is also used to quickly compute the load in each block by counting
the number of occupied slots in the metadata block.

\subsection{Operations}

\begin{algorithm}[t]
\centering
\caption{Insert (x, y)}
\label{alg:insert}
\begin{algorithmic}[1]
  \State $idx \gets h_0(x)$ \Comment{Compute the block index in level 1}
  \State $fp \gets \mathscr{F}(x)$  \Comment{Compute the fingerprint for key}
  \State $mask \gets \Call{Metadata\_Mask}{\mbox{lv1\_metadata}[idx], \texttt{EMPTY}}$
  \Comment{Compute a vector identifying empty slots in the block}
  \State $count \gets \Call{popcount}{mask}$  \Comment{Compute the number of empty
  slots}
  \State $i \gets 0$
  \While{$i < count$}
  \State $slot \gets \Call{Select}{mask, i}$ \Comment{Compute the index of the
  next empty slot}
  \If {\Call{atomic\_cas}{\mbox{lv1\_metadata}[idx][slot], \texttt{EMPTY}, \texttt{RESERVED}}}
  \Comment{Atomically set the metadata slot before updating the table}
  \State $\mbox{lv1\_block}[idx][slot].key \gets x$
  \State $\mbox{lv1\_block}[idx][slot].val \gets y$
  \State $\mbox{lv1\_metadata}[idx][slot] \gets fp$
  \State \Return True
  \EndIf
  \State $i \gets i+1$
  \EndWhile
  \State \Return \Call{insert\_lv2}{$x,y,idx$} \Comment{Level 1 block is full.
  Try level 2}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\centering
\caption{Insert level2 (x, y)}
\label{alg:insertlv2}
\begin{algorithmic}[1]
  \Procedure{insert\_lv2}{$x, y, idx$}
    \State $idx1 \gets h_1(x)$ \Comment{Compute primary and secondary block
    indexes in level 2}
    \State $idx2 \gets h_2(x)$
    \State $fp1 \gets \mathscr{F}_1(x)$  \Comment{Compute primary and secondary
    fingerprints for the key}
    \State $fp2 \gets \mathscr{F}_2(x)$

    \State
    \State $mask1 \gets \Call{Metadata\_Mask}{\mbox{lv2\_metadata}[idx1], \texttt{EMPTY}}$
    \Comment{Compute a vector identifying empty slots in primary and
    secondary blocks}
    \State $mask2 \gets \Call{Metadata\_Mask}{\mbox{lv2\_metadata}[idx2], \texttt{EMPTY}}$
    \State $count1 \gets \Call{popcount}{mask1}$  \Comment{Compute the number of empty
    slots in primary and secondary blocks}
    \State $count2 \gets \Call{popcount}{mask2}$

    \State
    \If {$count1 < count2$}
    \State $idx1 \gets idx2$
    \State $fp1 \gets fp2$
    \State $mask1 \gets mask2$
    \State $count1 \gets count2$
    \EndIf

    \State $i \gets 0$
    \While{$i < count1$}
    \State $slot \gets \Call{Select}{mask1, i}$ \Comment{Compute the index of the
    next empty slot}
    \If {\Call{atomic\_cas}{\mbox{lv2\_metadata}[idx1][slot], \texttt{EMPTY}, \texttt{RESERVED}}}
    \Comment{Atomically set the metadata slot before updating the table}
    \State $\mbox{lv2\_block}[idx1][slot].key \gets x$
    \State $\mbox{lv2\_block}[idx1][slot].val \gets y$
    \State $\mbox{lv2\_metadata}[idx1][slot] \gets fp1$
    \State \Return True
    \EndIf
    \State $i \gets i+1$
    \EndWhile
    \State \Return \Call{insert\_lv3}{$x,y,idx$} \Comment{Level 2 block is full.
    Try level 3}
  \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\centering
\caption{Insert level3 (x, y)}
\label{alg:insertlv3}
\begin{algorithmic}[1]
  \Procedure{insert\_lv3}{$x, y, idx$}
    \While {\Call{atomic\_test\_set}{\mbox{lv3\_locks}[idx], 0, 1}} \Comment{Try
    and grab a lock on the list head}
    \EndWhile
    \State $node \gets \Call{new\_node}{\null}$ \Comment{Create a new node}
    \State $node.key \gets x$
    \State $node.val \gets y$
    \State $node.next \gets \mbox{lv3\_nodes}[idx].head$ \Comment{Make new node
    the head of the list}
    \State $\mbox{lv3\_nodes}[idx].head \gets node$
    \State $\mbox{lv3\_locks}[idx] \gets 0$  \Comment{Release the lock}
  \EndProcedure
\end{algorithmic}
\end{algorithm}

Here we explain how to perform single-threaded operations in \sysname. Later
in~\Cref{multithreading}, we explain how to make these operations thread-safe.

\mab{Can we move the pseudocode to an appendix?}


\para{Inserts}
%
We first try to insert the key-value pair in level 1. We hash the key using
$h_0(x)$ to determine a block in level 1. If there is an empty slot in the block
then we insert the key-value pair and store the fingerprint in the
corresponding slot in the level 1 metadata. See the pseudocode
in~\Cref{alg:insert}.

If the block in level~1 is full, then we try to insert the key in level~2.  In
level~2, we use power-of-two-choice hashing to determine the block. We hash the
key twice and pick the emptier block. Similar to level~1, if there is an empty
slot in one of the blocks then we insert the key-value pair and store the
fingerprint in the corresponding slot in the level~2 metadata. See the
pseudocode in~\Cref{alg:insertlv2}.

Finally, if both the blocks in level~2 are full, then we insert the key in level~3. We use the hash function from level~1 ($h_0(x)$) to determine the linked list
to insert the key-value pair and insert at the head of the
linked list. See the pseudocode in \Cref{alg:insertlv3}.
  
\para{Queries}
%
Similar to the insert operations, we perform queries starting from
level 1 and moving to levels 2 and 3 if we do not find the key in the
previous level.

During a query, we determine the block in a level in the same way as
we do during the insert. In level 1 and 3, there is only one block to
check and we use use hash function $h_0(x)$ to determine the block.  In level 2,
the key can be present in either of the primary or the secondary block.
Therefore, we also perform a check in the secondary block if the key is not
found in the primary block.
 
Once we determine the block, we then perform a quick check to see if the
fingerprint of the queried key is present in the metadata of the block. Checking
the fingerprint requires a single memory access as all the fingerprints in a
given block fit inside a cache line.
%
If the fingerprint is not found in the metadata of the block then we can
terminate the query at that level and move to the next level. Otherwise, if one
or more fingerprint matches are found in the metadata of the block we then
perform a complete key match in the table for all possible matches and return a
pointer to the value if a key match is found.

If we are in level 3 during a query, we perform a linear search through the
linked list to find the key. However, buckets in level 3 are almost always empty
(<{}<1\% please refer to~\Cref{tab:key-dist}) and therefore we rarely have to
perform the linear search through the linked list.

\para{Deletions}
%
Deletions are performed similarly to queries. We first look
for the key starting from level 1 and then proceed to levels 2 and 3 if the key is not yet
found. Once the key is found, we first reset the
corresponding fingerprint in the metadata and then reset the key-value pair slot
in the table.

The pseudo-code for the query and remove operations follow the similar approach
as the insert operation pseudo-code. Therefore, they are omitted from the paper
to avoid redundancy.\mab{Do we need this comment about the pseudocode being redundant? Not if we don't have the other pseudocode until the appendix, I think.}



==> backups/intro.tex <==
% !TEX root =  main.tex

\section{Introduction}

%\alex{Do we want some sort of throwaway intro line here?}

\mfc{Please fix this intro sentence}


Future generations of storage will require high-performance DRAM and
PMEM hash tables.  
DRAM hash table performance is primarily determined by the number of cache lines
accessed during queries and updates.  PMEM adds a further constraint: writes are
more expensive than reads~\cite{pmem-measurements}, so it is critical to
minimize not only the number of cache lines read but the number of cache lines
dirtied per insertion.  Designing both \alex{suggest replacing ``both'' with ``high performance''} DRAM hash tables~\cite{LiAn14, Pheatt08,
NielsenKa16,fagin1979extendible,MaierSaDe16,ChandramouliPrKo18,F14,maier2019dynamic}
and PMEM hash tables~\cite{MaierSaDe19, MaierSaDe16,
LuHaWa20,pfht,path-hashing,level-hashing,cceh,nvc-hashmap,LeeEtAl19-Recipe,HuCh21,phprx}
is an active field of research.

% \mfc{the abstract seems stronger than the following}

% In this paper, we build \textbf{\sysname}, a new hash table that exhibits very
% high performance in both DRAM and PMEM.  \sysname achieves good cache locality
% on both queries and updates by simultaneously guaranteeing two properties:
% \defn{referential stability} and \defn{low associativity}.
% \mab{To improve: put in the sentence from the abstract that says that these properties are what leads to universal performance on both types of hardware and across a range of workloads. maybe just copy the same sentence.}


In this paper, we build \textbf{\sysname}, a new hash table that exhibits very
high performance in both DRAM and PMEM. In PMEM, it is also crash safe.
\sysname  simultaneously guarantees two properties, \defn{referential stability} and \defn{low associativity},
which helps it to achieve good cache locality on both queries and updates,  for workloads ranging from read-heavy to  write-heavy, and in both DRAM and PMEM.
These two properties also help to alleviate  most of the difficulties in achieving crash consistency.
% Yet, as we explain below, there is a tension between these two properties, and 
Previous hash-table designs have satisfied at most
one of these properties at a time.
\mab{this paragraph was previously very weak. Hopefully it is stronger now. Is it too repetitive? A little repetition doesn't bother me, and too much is better than too little.}




% MAB: paragraph from abstract.
% We begin by identifying two properties of hash tables,
% \emph{stability} and \emph{low associativity}, that when achieved
% simultaneously can result in strong performance in both DRAM and PMEM
% while simultaneously removing most of the difficulties in achieving
% crash consistency.  A hash table is \defn{stable} if it guarantees
% that the position where an element is stored will not change until
% either the element is deleted or the table is resized. A hash table
% has \defn{low associativity} if the maximum number of locations where
% an element is permitted to reside is small.  There is a tension
% between these two properties, and existing hash tables achieve at most
% one of these properties.



A hash table is said to be \defn{stable} if the position where an element is
stored is guaranteed not to change until either the element is deleted or the
table is resized~\cite{sandersstability,originalstability,KnuthVol3}.
%\footnote{Stability is weaker than referential integrity, which requires that
%the item never move, even after the table is resized.}  MAB: deleting the
%footnote since it seems to be a weaker.
Stability offers a number of desirable properties.  For example, stability
enables simpler concurrency-control mechanisms and thus reduces the performance
impact of locking.  Moreover, since elements are not moved, writing is
minimized, which improves PMEM performance.

The \defn{associativity} of a hash table is the number of locations where an
element is allowed to be stored.\footnote{Associativity is often associated with
caches that restrict the locations an item may be stored in.  Here we refer to
\emph{data structural associativity}, which is a restriction on how many locations a
data structure may choose from to put an item in, even on fully associative
hardware.} The best known low-associative hash table is the cuckoo hash
table~\cite{Pagh:CuckooHash,PaghRo01}.  In the original design, each element has
exactly two locations in the table where it is allowed to be stored, meaning
that the associativity is 2.  Low associativity yields a different set of desirable
properties---most importantly, it helps search costs. Thus, searching for an
element in a cuckoo hash table is fast, because there are only two locations in
the table to check.  In addition, low associativity can reduce the size of metadata, further
improving cache locality; see \Cref{sec:design}.


In combination, stability can be used to achieve high insertion
throughput (especially in PMEM, where writes are expensive), and low associativity can be use to achieve high query
throughput.
Stability means that locking and concurrency-control mechanisms can be simplified leading to better multithreaded scaling and simpler designs for crash consistency.
\mab{This paragraph was very weak.  Is it better now?}

Unfortunately, there is a tension between stability and low associativity.  If a
hash table has associativity $\alpha$, and elements cannot move once they are
inserted, then an unlucky choice of $\alpha$ locations for $\alpha$ elements can block a
$(\alpha+1)$st element from being inserted.  As $\alpha$ decreases, the probability of
such an unlucky event increases.  Cuckoo hashing reduces the probability of these bad
events by giving up stability via
\defn{kickout chains}, which are chains of elements that displace each other from one
location to another. Practical implementations~\cite{LiAn14} generally increase
the number of elements that can be stored in a given location---and thus the
associativity---to reduce the kickout-chain length and increase the
maximum-allowed \defn{load factor}, i.e, the ratio of the total number of
keys in the table to the overall capacity of the table.
To date, hash tables have had to choose between stability (e.g., chaining),
low associativity (e.g., cuckoo) or neither
(e.g., Robin Hood~\cite{CelisLaMu85,AmbleKn74}).


\para{Results}
In this paper, we introduce Iceberg hashing and its implementation, \sysname.
We prove that Iceberg hashing simultaneously achieves stability and low associativity. 
Iceberg hashing is the first hash-table design to achieve both properties.
These guarantees give \sysname excellent performance on both DRAM and PMEM and for workloads ranging from read-heavy to  write-heavy.
Specifically, \sysname accesses very few cache lines, both for queries and insertions, has low CPU cost, and has 
high load factor, with high probability.
Stability and low associativity enable simpler concurrency mechanisms, so that \sysname achieves nearly linear scaling with the number of threads, and it is crash safe on PMEM.

% {\color{gray}
% In this paper, we introduce Iceberg hashing and its implementation, \sysname.  
% We show that Iceberg hashing offers strong theoretical guarantees and demonstrate that these guarantees translate to excellent performance on DRAM and PMEM in workloads ranging from read-heavy to  write-heavy.
% Further, our PMEM implementation is crash safe.
% Moreover, \sysname achieves nearly l

% crash safety on PMEM. 

% We prove that Iceberg hashing simultaneously achieves stability and low associativity.  We first prove that
% \sysname accesses very few cache lines, both for queries and insertions, has low CPU cost, and has 
% high load factor, with high probability.

% }

% We show how to build an Iceberg hash table on a
% multi-core system and we establish that our design offers excellent performance.
% Our hash table is designed to perform well on both DRAM and PMEM and to offer
% crash safety on PMEM. 

In building \sysname, based on our Iceberg hash table, we offer the following design contributions:
\begin{enumerate}
\item We show how to augment an asymptotically optimal indexing
  scheme
     % given in Bender et al.~\cite{iceberg}
     % MAB: removing references to arXiv
  with a practical metadata scheme that is adapted it to practical hardware
  constraints.
\mab{Do we still want this ``augment'' phrasing? }
  The metadata scheme is small enough that the metadata
  for a bucket fits in a cache line, improving query performance and enabling nearly lock-free concurrency,
  i.e., locks are needed for
  a very small fraction of insertions and for resizing.
\item A highly concurrent and thread-safe implementation of Iceberg
  hashing.  \sysname can scale almost linearly with increasing threads
  in both DRAM and PMEM experiments.
\item Fenceless crash safety on PMEM.  Achieving crash-safety on PMEM
  often requires controlling the order in which cache lines get
  flushed to persistent storage, e.g., to ensure that an undo-log
  entry gets persisted before the changes to the hash table get
  persisted.  Since insertions in our hash table modify only a single
  cache line, we can achieve crash safety by simply persisting that
  cache line.
\item A simple, high-performance and concurrent technique for
  efficiently resizing Iceberg hash tables in a lazy online manner,
  thus reducing the worst-case latency of insertions.
\end{enumerate}

\para{Performance}
We evaluated \sysname both in DRAM and in PMEM.
In all but one experiment, \sysname outperforms libcuckoo~\cite{LiAn14} and
TBB~\cite{Pheatt08} in DRAM and Dash~\cite{LuHaWa20} in PMEM.

In particular,
\begin{enumerate}
  \item \textbf{DRAM inserts:} \sysname is  up to $2.3\times$ faster than
    libcuckoo and $9.1\times$ faster than TBB.
  \item \textbf{DRAM queries:} \sysname is  up to $1.7\times$ faster than
    libcuckoo and $2.6\times$ faster than TBB.
  \item \textbf{DRAM deletions:} \sysname is slower (50\%) for
    deletions than libcuckoo but it is up to $5.3\times$ faster than TBB.
  \item \textbf{DRAM YCSB:} \sysname is faster than libcuckoo and
    TBB for three different YCSB workloads. It is up to $3.9\times$ faster for
    workload A, $2.7\times$ faster for workload B, and $2.8\times$ faster for
    workload C.
  \item \textbf{PMEM inserts/queries/deletions:} \sysname is between
    $1.1\times$ to $1.8\times$ faster than Dash.
  \item \textbf{PMEM YCSB:} \sysname is between $1.7\times$ to $1.8\times$
    faster than Dash for YCSB workloads A, B, and C on PMEM.
  \item \textbf{Tail Latency.} \sysname's worst case insertion latency while
    resising is up to three orders of magnitude faster than libcuckoo and TBB.
  \item \textbf{Scalability.} \sysname's performance grows between $13.5\times$
    to $14.1\times$ going from 1 to 16 threads compared to libcukoo that grows
    between $8.7\times$ and $11.3\times$ and TBB between $1.6\times$ and
    $13.4\times$ in DRAM.
  \item \textbf{Space.} \sysname has up to $1.4\times$ less peak memory usage
    (Max RSS) compared to libcuckoo across resizes.
\end{enumerate}

\para{Roadmap}
%
In the rest of the paper, we discuss the various hash table designs
in~\Cref{sec:model}. In~\Cref{sec:theory}, we give an overview of Iceberg
hashing and theoretical guarantees.
In~\Cref{sec:design,resizing,multithreading,sec:pmem}, we present our
implementation of \sysname in DRAM and PMEM. \Cref{sec:eval} evaluates \sysname
and compares it with other hash tables.
%
We discuss related work in~\Cref{sec:related}.
%and conclude
%in~\Cref{sec:conclusion}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> backups/model.tex <==
% !TEX root =  main.tex

\section{Hash Table Design Goals}
\label{sec:model}

% Hash tables have struggled for decades to balance the costs of queries
% and insertions~\cite{Knuth63,Knuth98,CelisLaMu85,PaghR01}.
% As memory speeds have lagged behind CPU speeds, the bottleneck
% has shifted from CPU costs and to memory-access
% costs~\cite{PaghR01}.  Multi-core systems now mean that hash tables
% must support high degrees of concurrency.  Persistent memory amplifies
% memory-access costs, making it even more important to design hash
% tables that access only a few cache lines per operation, and also have
% higher write costs than read costs, which shifts the whole design
% space to favor reads over writes~\cite{pmem-measurements}.  Finally,
% persistent memory also requires hash tables to deal with crash safety.


In this section, we explore how classic hash-table schemes
interact with modern hardware in order to understand the design of Iceberg hashing and \sysname.  Specifically, we consider
chaining~\cite{Knuth98}, 
linear probing~\cite{Knuth63}, Robin Hood hashing~\cite{CelisLaMu85,AmbleKn74},
and cuckoo hashing~\cite{PaghR01}.  We evaluate them on
four criteria:
\begin{itemize}[noitemsep]
%\itemsep0em 

  \item The number of cache lines read during queries and updates.
  \item The number of cache lines written during updates, since writes
    are especially expensive on PMEM.
  \item The overhead of supporting concurrent operations.
  \item The overhead of ensuring crash safety on
    persistent memory.
\end{itemize} 

\para{Chaining} In a chaining hash table, items are hashed
to a slot in the table and added to that slot's linked list.  The table
can be resized to maintain a constant average linked list size
(typically between ${1}/{2}$ and 2).  
%\mab{Move to next paragraph somewhere: By reusing the linked-list
% nodes during a resize, chaining can offer referential integrity,
% i.e. an item never moves after it is inserted into the table, which
% means it is safe to expose pointers to elements of the table.}
Chaining can be made concurrent by locking each table entry or by
using lock-free linked lists, although deletes must deal with the
memory-reclamation challenges that all lock-free data structures
face~\cite{HartMcDe07}, and locking may still be needed to coordinate
resizes.

Chaining has drawbacks that keep it from being used in
high-performance hash tables except when stability is absolutely essential.\footnote{Stability is a necessary condition for referential integrity, which 
  means that an item never moves after it is inserted into the table,
  which means it is safe to expose pointers to elements of the
  table. Chaining hash table can guarantee referential integrity by
  reusing the linked-list nodes during a resize.  } First, a
linked-list traversal typically entails one cache miss to look up the
list head plus a cache miss per node.  Furthermore, these memory
accesses are dependent, so they cannot be performed in parallel.  On
persistent memory, each insertion needs to modify at least two cache
lines (one for the new linked-list node and one for the pointer to the
new node).  Although crash safety can be achieved by first making the
new node durable and then the pointer to the new node, a fence is needed
between the writes.  Chaining also requires a crash-safe allocator for the
nodes.  Finally, the space overhead of the table and linked-list
pointers can be substantial.  
%For example, if keys and value are each a word, and we target the
%number of linked lists to be equal to the number of elements in the
%hash table, then the space overhead is $2\times$.

\para{Linear probing} Linear probing is an instance of open
addressing~\cite{knuth:texbook}.  With open addressing, the hash table consists of an array
of slots.  Items are stored in the slots.  The slot for each item is
chosen via one or more hash functions and a collision-resolution
scheme.  Essentially all modern high-performance hash tables use some
form of open addressing.

In linear probing, each item is hashed to a slot.  The algorithm then
scans forward through the slots until it finds the first empty slot,
where it places the item.  This greatly improves locality, and insertions
modify only a single slot.  Deletions are usually implemented by tombstones,
i.e., by marking the item as deleted.  Concurrency can be implemented
by locking ranges of slots and using a hand-over-hand locking style.
Some variants are even lock-free~\cite{MaierSaDe19}.

The main disadvantage of linear probing is that operations become
slower as the table fills, because the distance that must be scanned
for insertions or lookups grows~\cite{Knuth63,BenderKuKu22}.  For this reason, many linear-probing
hash tables resize the table when the fraction of occupied slots
reaches some threshold, such as 75\%, meaning that space overhead is
always at least 33\%.  Also, lock-free implementations
often~\cite{NielsenKa16} let tombstones accumulate until the table is
resized, rather than reusing the slots, making operations even slower.

\mab{Need citations for paragraph.}
Other classic variants of open addressing, such as quadratic probing
or double hashing, may reduce the number of slots that must be probed
but reduce cache locality.

\para{Robin Hood hashing} Robin Hood hashing~\cite{CelisLaMu85} is a
general technique for improving query performance in open-addressing
hash tables by rearranging elements on insertion.  The Robin-hood
technique can be applied to many of the classic open-addressing
schemes.  For brevity we describe only the linear-probing variant.
% and also makes it more difficult to achieve lock freedom.
With Robin-hood linear probing, during an insert, we maintain the
invariant that items are stored in sorted order by hash value.  This
means, on the one hand, that queries can stop early if they find a
larger hash value than their target, but on the other hand, that runs
of items may need to be shifted to make room for an insertion, in the
style of insertion sort.

Robin Hood hashing can be made concurrent by using locks on ranges of
slots (with hand-over-hand locking).  Most implementations are not lock free because
insertions  temporarily remove elements
from the hash array as they get shifted. 
Reshuffling elements also
makes it more complex and expensive to maintain crash safety because it requires the use of fences.\mab{please verify that it's fences that make it more expensive.}  Finally, shuffling
elements increases the amount of data written per insert, which is undesirable on persistent memory.

\para{Cuckoo} Cuckoo hashing~\cite{PaghR01} shares with Robin Hood
hashing the notion of displacing items to make room for insertions.
It differs from previous hashing schemes in that it reduces the
associativity of the hash table to a constant, at the cost of reduced
cache locality, especially during inserts.  In a cuckoo hash table,
the slots are grouped into buckets (of size 4 in a typical
implementation).  Each item is hashed to two buckets.  If either
bucket has a free slot, then the item is stored there.  If not, then
the hash table selects an item in one of the buckets and \defn{kicks}
it to its alternate bucket.  This kicking process may repeat, which is
why cuckoo hash tables slow down as they become full.

The kicking process is particularly expensive on persistent memory,
because of high write costs~\cite{pmem-measurements}.  Furthermore,
hand-over-hand locking during the kicks can result in result in
deadlock.  One workaround is to precompute the entire kicking
sequence, then lock all the involved buckets from left to right, then
check that the sequence of kicks will still work, and then finally
perform the kicks.  This technique can also be used to make the table
crash safe (i.e. by applying the kicking chain in reverse, with fences
between every step, so that every key is always in at least one slot
of the table), but the fences may introduce overheads.

\para{Summary}
In conclusion, prior hash-table designs have faced trade-offs between
query performance and insertion performance.  They can incur extra
concurrency-control costs, perform possibly 
many writes, making them slow on persistent memory, or require
multiple fence instructions and additional mechanisms in order to be
made crash safe.

We have picked representative examples from major hash-table design
families to demonstrate that there is a tension between achieving low
associativity and stability and that this tension has performance
consequences.  These analyses apply more broadly; see \Cref{sec:related}.
For example, Hopscotch hashing~\cite{HerlihyShTz08} faces many of the
same issues as Robin-hood hashing.  And, although there is a huge body
of work on making these structures fast, concurrent, and, recently,
crash safe, these techniques often introduce complexity or overheads.
The goal of this paper is to create a hash table in which concurrency
and crash safety fall out of the stable, low-associativity design with
little to no additional complexity or overheads.



==> backups/theory.tex <==
% !TEX root =  main.tex

\section{Iceberg Hashing}
\label{sec:theory}

In this section, we describe the theoretical basis for \sysname.
In~\cite{iceberg}, Bender et al.\ introduced the
the Iceberg hash table and showed that it is stable and has low associativity.
They show how to achieve constant-time operations, one I/O (cache line miss) per
operation, and high load factors.

Iceberg hashing is a front yard/backyard hashing scheme~\cite{arbitman2010backyard,peterson57,BenderFaGo18, goodrich2011fully, goodrich2012cache}.
Most inserted items land in the front yard.  When there is no room for an element in the front
yard, it get inserted into the backyard.  Only a small percentage
of elements make it to the backyard, so the data structure used in the
backyard need not be as space efficient as that used in the front
yard, but it needs to be able to handle all items that arrive, whereas
the front yard needs to be highly space efficient but only need
work with a reasonable probability.

This general setup covers many choices of front yard design and
backyard design, as well as rules for moving items from the
backyard to the front yard.  Until recently, there were no techniques
for bounding the number of items that land in the backyard, thus all
systems used a rule to sometimes move items to the front yard.  Such
rules preclude stability in the hash table.  
%Indeed, if an adversary knows which items are in the front yard and
%which are in the backyard, they can drive the system to store more
%and more items in the (inefficient) backyard.  
A critical technical innovation of Iceberg hash
tables is a simple front-yard design that bounds
the number of items in the backyard, even under dynamic loads when
items can be inserted, deleted and reinserted.  This makes Iceberg hash
tables stable.

Specifically, consider a hash table with a front yard consisting of an
array of length $m$ broken into $n$ buckets of size
$m/n = h\approx \log m$. Items are hashed to a single bucket and may
be placed in any slot in their bucket. Once inserted, items are not moved
until they are deleted. For now, leave the backyard design as a black
box. We have the following bound on the number of items which are
present in the backyard at any point in time.

\begin{lemma}[Iceberg lemma~\cite{iceberg}]
   Consider a backyard hash table whose front yard consists of $n$ buckets,
   into which a sequence of insertions and deletions are performed, such that
   there are at most $m=hn$ items present at any given time. If each bucket has
   at least $h + \tau_h$ slots, where $\tau_h = k\cdot(h\log{h})^{1/2}$ and
   $h\leq\polylog{m},$ then at any point there are at most $n/\poly{h}$ items
   in the backyard, w.h.p. in $m$.
\end{lemma}


\begin{theorem}
Let $m, h, j$ be variables with $h \le n^{1/4} / \sqrt{\log n}$ and $j \le \sqrt{h}$. Consider a sequence of $\poly(m)$ insertions/deletions of balls from a universe $U$, where each $x \in U$ is assigned a random bin $h(x) \in [m]$, and where there are at most $n = hm$ balls present at a time. Suppose that whenever a ball $x$ is inserted, we place it using the following rule: if bin $h(x)$ currently has no more than $h + j\sqrt{h + 1} + 1$ balls then $x$ gets inserted into the bin, and otherwise, $x$ gets placed into a \defn{backyard}. Then, at any given moment, the number of balls in the backyard is $O(n / 2^{\Omega(j^2)} + n^{3/4}\sqrt{\log n})$ with probability $1 - 1 / \poly(n)$. 
\end{theorem}
\begin{proof}
For the sake of analysis, partition the bins into $K = \sqrt{n}$ collections $\mathcal{B}_1, \ldots, \mathcal{B}_{K}$ each of which contains $m / K$ bins. For each time $t$ and bin collection $\mathcal{B}_i$, define $R_{t, i}$ to be the set of balls $x$ that are present at time $t$ and satisfy $h(x) \in \mathcal{B}_i$. By a standard application of Chernoff bounds, we can deduce that, for any fixed $i, t$ we have 
\begin{equation}
|R_{i, t}| \le n / K + O(\sqrt{(\log n) \cdot n / K}) \le \sqrt{n} + O(n^{1/4}\sqrt{\log n})
\label{eq:rit}
\end{equation}
with high probability in $n$ (i.e., with probability $1 - 1 / \poly(n)$). Applying a union bound over all $i, t$, we find that \eqref{eq:rit} holds with high probability in $n$ for all $i, t$ simultaneously. Consider any possible outcome $R$ for the sets $\{R_{i, t}\}$, where the only requirement on $R$ is that \eqref{eq:rit} holds for all $i, t$;  we will show that if we condition on such an $R$ occurring, then the size of the backyard is $O(n / 2^{\Omega(j^2)} + n^{3/4}\sqrt{\log n})$ with high probability in $n$.

Consider some time $t$, and let $X_i$ be the number of balls that are in the backyard at time $t$ and that satisfy $h(x) \in \mathcal{B}_i$. Observe that the conditional variables $X_1 | R, X_2 | R, \ldots, X_{K} | R$ are independent (since $R$ fully determines which $x$ and $i$ satisfy $h(x) \in \mathcal{B}_i$). Thus, if we define
$$X | R := \sum_{i = 1}^{K} X_i | R,$$
then $X | R$ is a sum of independent random variables, each of which is (by \eqref{eq:rit}) deterministically in the range $[0, O(\sqrt{n})]$. We can therefore apply a Chernoff bound to $X | R$ to deduce that
$$\Pr[X | R \le \E[X | R] + O(\sqrt{Kn\log n})] \ge 1 - 1 / \poly(n),$$
Recalling that $K = \sqrt{n}$, we conclude that $X | R \le \E[X | R] + O(n^{3/4}\sqrt{\log n})$ with high probability in $n$. 

To complete the proof, it suffices to bound $\E[X | R]$ by $O(n / 2^{\Omega(j^2)})$. For this, in turn, it suffices to show that each ball $x$ present at time $t$ (there are up to $n$ such balls) satisfies
\begin{equation}
\Pr[x \text{ in backyard} \mid R] \le 1 / 2^{\Omega(j^2)}.
\label{eq:indball}
\end{equation}
To prove \eqref{eq:indball}, consider a ball $x$ that hashes to some collection $\mathcal{H}_i$. At the previous time $t_0 < t$ that $x$ was inserted, we have by \eqref{eq:rit} that there were at most $\sqrt{n} + O(n^{1/4} \sqrt{\log n})$ balls present that hashed to $\mathcal{H}_i$ (i.e., balls in the set $R_{i, t_0} \setminus \{x\}$); each of these balls has probability $K / m = K / (n / h) = Kh / n$ of hashing to the same bin as $x$, meaning that the number $Y$ of balls that hash to the same bin as $x$ at time $t_0$ satisfies
$$\E[Y | R] \le \frac{Kh\sqrt{n} + O(Khn^{1/4}\sqrt{\log n})}{n} = h (1 + \sqrt{\log n} / n^{1/4}) \le h + 1.$$
The random variable $Y | R$ is just a sum of (up to) $n^{2/3} + O(n^{1/3} \sqrt{\log n})$ independent indicator random variables (one for each ball in $R_{i, t_0} \setminus \{x\}$). So by a Chernoff bound we have that
$$\Pr[Y \mid R \ge h + 1 + j \sqrt{h + 1}] \le 2^{-\Omega(j^2)}.$$ 
This implies \eqref{eq:indball}, which completes the proof. 
\end{proof}



The main consequence of this lemma is that this simple bucketed front yard
design can hold all but $n/\poly{h}$ items, and by design the front yard is
also stable.

Iceberg hashing allows any of several backyard designs.  For \sysname,
we have selected a hash table strategy based on the
power-of-2-choices. Specifically, it consists of an array of length
$O(n\log\log{n})$, divided into $n$ buckets of size $\omega(\log\log{n})$. \alex{Is the first $O$ supposed to be $\omega$ or the other way around?}
Items are hashed to two buckets and are placed into a slot in the bucket with
fewer items. The following result of V\"{o}cking provides a theoretical guarantee
that the backyard will not overflow.

\begin{theorem}[\cite{vocking2003asymmetry}]
   Consider an infinite balls-and-bins process with $n$ bins in which at each
   step a ball is either inserted using the power-of-2-choices algorithm or an
   existing ball is removed, such that there are at most $hn$ balls present at
   any given step. Then the maximum load of any given bin is $\ln\ln{n}/\ln{2}
   + O(h)$.
\end{theorem}

For the second level, $h$ \alex{$h$ is sort of ambiguous here.} is less than 1, so the number of overflowing
balls is quite small.  We store these balls in a third level that
uses a standard chaining hash table.  So few balls make it to the
third level that performance and space efficiency are not critical.

This design offers several benefits:
\begin{itemize}
  \item Such a table is stable, that is, items never move after they are inserted.
  \item The number of buckets an item can reside in is only 4 (1
    bucket in level 1, 2 in level 2, and one in level 3).
  \item Most queries are satisfied by searching in level 1, so the
    average number of buckets accesses per query is just over 1.
  \item The buckets are small, so the associativity of the scheme is
    $\log n + \log \log n$ (plus level 3, which is rarely used).  So
    we can encode the exact slot of an element  using $\log\log
    m$ bits.
\end{itemize}

%{\color{red}This section is not done. Here's an outline. Someone will need to finish this.
%\begin{itemize}
%\item Iceberg lemma stated in terms of backyard rather than exposed balls. What it has to do with stability.
%\item Single-choice dynamic bounds and power-of-2 choice dynamic bounds.
%\item
%Theoretical justification for our three-level design. Explain how our design is different from the theoretical design.What this has to do with low associativity. How our level II is different and why.
%\end{itemize}
%}


==> defines.tex <==
% !TEX root =  main.tex

%%%%%%%%%%%%
% Annotations for revisions
%%%%%%%%%%%%

\makeatletter
\newcommand{\InFloat}[2]{\@ifundefined{@captype}{#2}{#1}}
\makeatother

\newcommand{\marginparifpossible}[1]{\InFloat{{#1}}{\marginpar{#1}}}
\newcommand{\mymarginpar}[1]{\marginparifpossible{\sf \scriptsize \color{blue}{#1} }}
\newcommand{\rev}[2]{\mymarginpar{#1}{\color{blue}{#2}}}

\renewcommand{\mymarginpar}[1]{}
\renewcommand{\rev}[2]{\mymarginpar{#1}{{#2}}}



\renewcommand{\epsilon}{\varepsilon}

% \newcommand{\defn}[1]{\textit{#1}}
\newcommand{\defn}[1]{{\textit{\textbf{\boldmath #1}}}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{observation}[theorem]{Observation}

\makeatletter
\algrenewcommand\ALG@beginalgorithmic{\footnotesize}
\makeatother


\definecolor{magenta4}{rgb}{0.5625,0,0.5625}
\definecolor{green4}{rgb}{0,0.5625,0}
\definecolor{orange4}{rgb}{0.98,0.31,0.09}

\iffalse 
\newcommand{\rob}[1]{{\scriptsize \textcolor{pink}{Rob: {#1}}}}
\newcommand{\mfc}[1]{{\scriptsize \textcolor{orange4}{Martin: {#1}}}}

\newcommand{\mab}[1]{{\scriptsize \textcolor{red}{Michael: {#1}}}}

\newcommand{\alex}[1]{{\scriptsize \textcolor{magenta}{Alex: {#1}}}}
\newcommand{\prashant}[1]{{\scriptsize \textcolor{cyan}{Prashant: {#1}}}}
\newcommand{\joe}[1]{{\scriptsize \textcolor{blue}{Joe: {#1}}}}
\fi 

% see http://latexcolor.com to define more colors

\newcommand{\rob}[1]{\todo[size=\tiny,color=pink]{Rob: #1}}
\newcommand{\mfc}[1]{\todo[size=\tiny,color=orange]{MFC: #1}}
\newcommand{\mab}[1]{\todo[size=\tiny,color=green!40]{MAB: #1}}
\newcommand{\alex}[1]{\todo[size=\tiny,color=magenta]{Alex: #1}}
\newcommand{\prashant}[1]{\todo[size=\tiny,color=cyan]{Prashant: #1}}
\newcommand{\joe}[1]{\todo[size=\tiny,color=green!20]{Joe: #1}}

\newcommand{\robinline}[1]{\todo[inline,size=\tiny,color=pink]{Rob: #1}}
\newcommand{\mfcinline}[1]{\todo[inline,size=\tiny,color=orange]{MFC: #1}}
\newcommand{\mabinline}[1]{\todo[inline,size=\tiny,color=green!40]{MAB: #1}}
\newcommand{\alexinline}[1]{\todo[inline,size=\tiny,color=magenta]{Alex: #1}}
\newcommand{\prashantinline}[1]{\todo[inline,size=\tiny,color=cyan]{Prashant: #1}}
\newcommand{\joeinline}[1]{\todo[inline,size=\tiny,color=green!20]{Joe: #1}}



\newcommand{\fixme}[1]{\todo[size=\tiny]{#1}}

\newcommand{\TODO}{{\color{red}\bf TODO}}


%% comment the next few lines to remove all our comments
%\iffalse
\renewcommand{\rob}[1]{}
\renewcommand{\mfc}[1]{}
\renewcommand{\mab}[1]{}
\renewcommand{\alex}[1]{}
\renewcommand{\prashant}[1]{}
\renewcommand{\joe}[1]{}
\renewcommand{\robinline}[1]{}
\renewcommand{\mfcinline}[1]{}
\renewcommand{\mabinline}[1]{}
\renewcommand{\alexinline}[1]{}
\renewcommand{\prashantinline}[1]{}
\renewcommand{\joeinline}[1]{}
%\fi

\newcommand{\sysname}{\textsc{IcebergHT}\xspace}
\newcommand{\Sysname}{\textsc{IcebergHT}\xspace}
\newcommand{\dash}{Dash\xspace}
\newcommand{\cuckoo}{Cuckoo\xspace}
\newcommand{\tbb}{TBB\xspace}
\newcommand{\clht}{CLHT-LB-RES\xspace}

\newcommand{\poly}[1]{\textrm{poly}{(#1)}}
\newcommand{\polylog}[1]{\textrm{polylog}{(#1)}}

\newcommand{\para}[1]{\smallskip\noindent\textbf{#1.}}

\newcommand{\E}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}


==> plot-latency.tex <==
% !TEX root =  main.tex

\begin{figure}
   \centering
   \begin{subfigure}{\linewidth}
      \begin{tikzpicture}
         \begin{axis}[
               LatencyPlot,
               xmode=log,
            ]
            \addplot[IcebergStyle, mark=.] table[x=Latency_nsec, y=cdf] {data/ycsb_workloada_insert_cdf.csv};
         \end{axis}
      \end{tikzpicture}
      \caption{Insert}
      \label{insert-latency}
   \end{subfigure}\\
   \begin{subfigure}{\linewidth}
      \begin{tikzpicture}
         \begin{axis}[
               LatencyPlot,
               xmode=log,
            ]
            \addplot[IcebergStyle, mark=.] table[x=Latency_nsec, y=cdf] {data/ycsb_workloada_query_cdf.csv};
         \end{axis}
      \end{tikzpicture}
      \caption{Positive Query}
      \label{query-latency}
   \end{subfigure}%
\caption{Insertion, deletion, and lookup performance of hash tables in DRAM.}
\label{fig:latency-ycsb-dram}
\end{figure}

